MetaBEV: Solving Sensor Failures for BEV Detection and Map Segmentation

Perception systems in modern autonomous driving vehicles typically take inputs from complementary multi-modal sensors, e.g., LiDAR and cameras. However, in real-world applications, sensor corruptions and failures lead to inferior performances, thus compromising autonomous safety. In this paper, we propose a robust framework, called MetaBEV, to address extreme real-world environments involving overall six sensor corruptions and two extreme sensor-missing situations. In MetaBEV, signals from multiple sensors are first processed by modal-specific encoders. Subsequently, a set of dense BEV queries are initialized, termed meta-BEV. These queries are then processed iteratively by a BEV-Evolving decoder, which selectively aggregates deep features from either LiDAR, cameras, or both modalities. The updated BEV representations are further leveraged for multiple 3D prediction tasks. Additionally, we introduce a new M2oE structure to alleviate the performance drop on distinct tasks in multi-task joint learning. Finally, MetaBEV is evaluated on the nuScenes dataset with 3D object detection and BEV map segmentation tasks. Experiments show MetaBEV outperforms prior arts by a large margin on both full and corrupted modalities. For instance, when the LiDAR signal is missing, MetaBEV improves 35.5% detection NDS and 17.7% segmentation mIoU upon the vanilla BEVFusion model; and when the camera signal is absent, MetaBEV still achieves 69.2% NDS and 53.7% mIoU, which is even higher than previous works that perform on full-modalities. Moreover, MetaBEV performs fairly against previous methods in both canonical perception and multi-task learning settings, refreshing state-of-the-art nuScenes BEV map segmentation with 70.4% mIoU.

==> table/abla_switch_training.tex <==
\begin{table*}[t]
\footnotesize
\begin{center}
    \renewcommand{\tabcolsep}{5mm}
    \begin{tabular}{c | ccc  ccc  ccc }
    \toprule
        \multirow{2}{*}{Methods} & \multicolumn{3}{c}{Camera + Lidar} & \multicolumn{3}{c}{Total Camera Failure} & \multicolumn{3}{c}{Total Lidar Failure} \\
        \cmidrule[0.2mm](r){2-4}\cmidrule[0.2mm](r){5-7}\cmidrule[0.2mm](r){8-10}
        & mAP & NDS & mIoU & mAP & NDS & mIoU & mAP & NDS & mIoU \\
    \midrule
        TransFusion~\cite{bai-22cvpr-transfusion} & 67.3 & 71.2 & -- & 61.6 & 67.4 &-- &-- &-- &--  \\
        BEVFusion~\cite{liu-2022-bevfusion} & 68.5 & 71.4 & 62.7 & \gain{61.8} & \gain{67.5} & \gain{4.1} & \gain{0.5} & \gain{7.1} & \gain{36.7} \\
    \rowcolor{gray!15}        
        MetaBEV & 68.0 & 71.5 &  70.4 & 63.6 & 69.2 & 53.7 & 39.0 & 42.6 & 54.4 \\
    \bottomrule
    \end{tabular}
    % \vspace{8pt}
\end{center}
\vspace{-2mm}
\caption{\textbf{Experimental comparisons on extreme sensor missing.} \model\ is able to totally drop the features from the missing modalities for inference, while others cannot. We attempt to replace the missing features with zero in other works so that they can output results, which are colored as \gain{blue}.
\model\  still consistently outperforms prior works when facing extreme sensor absence.}
 \label{tab:missing_modal}
\vspace{-2mm}
\end{table*} 

